ETO:Efficient Transformer-based Local Feature Matching by Organizing Multiple Homography Hypotheses

We tackle the efficiency problem of learning local feature matching. Recent advancements have given rise to purely CNN-based and transformer-based approaches, each augmented with deep learning techniques. While CNN-based methods often excel in matching speed, transformer-based methods tend to provide more accurate matches. We propose an efficient transformer-based network architecture for local feature matching. This technique is built on constructing multiple homography hypotheses to approximate the continuous correspondence in the real world and uni-directional cross-attention to accelerate the refinement. On the YFCC100M dataset, our matching accuracy is competitive with LoFTR, a state-of-the-art transformer-based architecture, while the inference speed is boosted to 4 times, even outperforming the CNN-based methods. Comprehensive evaluations on other open datasets such as Megadepth, ScanNet, and HPatches demonstrate our method's efficacy, highlighting its potential to significantly enhance a wide array of downstream applications.

==> tables/1600.tex <==
\begin{table}[!t]
% \vspace{-0.6cm}

\tabcolsep 4pt
\footnotesize
% \normalsize

\centering
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{3}{c}{Pose estimation AUC}      \\ \cline{2-4} 
       & @5\textdegree            & @10\textdegree           & @20\textdegree         \\ \hline
\multicolumn{1}{l|}{LoFTR 640 Megadepth}                                        & 57.5          & 71.2          & 80.8        \\
\multicolumn{1}{l|}
{ETO 640 Megadepth}              & 51.7          & 66.6          & 77.4         \\ \hline
\multicolumn{1}{l|}{LoFTR 640 ScanNet}              & 21.4          &    40.3       & 57.2       \\
\multicolumn{1}{l|}{ETO 640 ScanNet}                                                         & 20.1 & 40.4 & 59.8  \\ \hline
\multicolumn{1}{l|}{LoFTR 1600 Megadepth}                                        & 9.7          & 17.0          & 25.2        \\
\multicolumn{1}{l|}
{ETO 1600 Megadepth}              & \textbf{62.4}          & \textbf{75.1}          & \textbf{83.8}         \\ \hline
\multicolumn{1}{l|}{LoFTR 1600 ScanNet}              & 2.3          &    5.3       & 9.5       \\
\multicolumn{1}{l|}{ETO 1600 ScanNet}                                                         & \textbf{22.2} & \textbf{42.7} & \textbf{61.4}  \\
\bottomrule
\end{tabular}
% \vspace{-0.3cm}
\caption{Evaluation for pose estimation on higher resolusion.}
\vspace{-0.3cm}
\label{tab:1600}

\end{table}

==> tables/megadepth_new.tex <==
\begin{table}[!t]
% \vspace{-0.3cm}

\tabcolsep 4pt
\footnotesize
% \normalsize

\centering
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Pose estimation AUC} & average time     \\ \cline{2-5} 
       & @5\textdegree            & @10\textdegree           & @20\textdegree  &  ms        \\ \hline
\multicolumn{1}{l|}{ASpanFormer}                                & 58.6    & 72.2    &  81.7   & 158.5  \\
\multicolumn{1}{l|}{Quadtree}&                                58.6     &    72.1       &    81.5       &   147.6       \\
\multicolumn{1}{l|}{LoFTR}                                           & 57.5          & 71.2          & 80.8     & 93.2     \\
\multicolumn{1}{l|}{SuperPoint+LightGlue}                                        & 51.5          & 67.7          & 78.9  & 64.2        \\
\multicolumn{1}{l|}{SuperPoint+LightGlue*}                                        & 47.1          & 64.0          & 77.3  & 26.9        \\
\multicolumn{1}{l|}
{SuperPoint+SuperGlue}              & 43.2          & 60.0          & 72.8    & 43.9      \\ 
\multicolumn{1}{l|}{Superpoint+search}              & 28.8          &    43.4       & 56.6  &  23.7      \\
\hline
\multicolumn{1}{l|}{PATS}              & 61.1          &    74.2       & 83.1  &  1475.9      \\
\multicolumn{1}{l|}{Efficient LoFTR}              & 59.2          &    72.6       & 81.8  &  56.9      \\
\hline
\multicolumn{1}{l|}{Ours}                                                         & 51.7 & 66.6 & 77.4 &\textbf{21.0} \\
\bottomrule
\end{tabular}
% \vspace{-0.3cm}
\caption{More complete evaluation on Megadepth for outdoor pose estimation. To be mentioned that our paper is contemporaneous with the Efficient LoFTR. And while PATS gets extremely good results, it is almost 100 times slower than our method.}
% \vspace{-0.6cm}
\label{tab:megadepth}

\end{table}

==> tables/yfcc_pose.tex <==
\begin{table}[!t]
% \vspace{-0.6cm}

\tabcolsep 4pt
\footnotesize
% \normalsize

\centering
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Pose estimation AUC} & average time     \\ \cline{2-5} 
       & @5\textdegree            & @10\textdegree           & @20\textdegree  &  ms        \\ \hline
\multicolumn{1}{l|}{ASpanFormer~\cite{aspanformer}}                                & 44.5    & 63.5    &  78.1   & 155.5  \\
\multicolumn{1}{l|}{Quadtree~\cite{quadtree}}                                     &     44.7      &   63.9        &      78.2 & 159.4     \\
\multicolumn{1}{l|}{LoFTR~\cite{loftr}}                                           & 44.7          & 63.6          & 78.3     & 96.3     \\
\multicolumn{1}{l|}{SP~\cite{superpoint}+LG~\cite{lightglue}}                                        & 36.1          & 56.2          & 73.1  & 60.8        \\
\multicolumn{1}{l|}{SP~\cite{superpoint}+LG*~\cite{lightglue}}                                        & 29.2          & 48.8          & 67.0  & 27.2        \\
\multicolumn{1}{l|}
{SP~\cite{superpoint}+SG~\cite{superglue}}              & 29.7          & 49.6          & 67.9    & 48.7      \\ 
\multicolumn{1}{l|}{SP~\cite{superpoint}+search}              & 14.0          &    27.0       & 42.2  &  24.6      \\
\hline
\multicolumn{1}{l|}{Ours}                                                         & \textbf{44.8} & \textbf{64.0} & \textbf{78.8} &\textbf{22.1} \\
\bottomrule
\end{tabular}
% \vspace{-0.3cm}
\caption{Evaluation on YFCC100M~\cite{yfcc100m} for outdoor pose estimation.}
% \vspace{-0.3cm}
\label{tab:yfcc}

\end{table}
